KPM-Bench: A Kinematic Parsing Motion Benchmark for Fine-grained Motion-centric Video Understanding

Despite recent advancements, video captioning models still face significant limitations in accurately describing fine-grained motion details and suffer from severe hallucination issues. These challenges become particularly prominent when generating captions for motion-centric videos, where precise depiction of intricate movements and limb dynamics is crucial yet often neglected. To alleviate this gap, we introduce an automated annotation pipeline that integrates kinematic-based motion computation with linguistic parsing, enabling detailed decomposition and description of complex human motions. Based on this pipeline, we construct and release the Kinematic Parsing Motion Benchmark (KPM-Bench), a novel open-source dataset designed to facilitate fine-grained motion understanding. KPM-Bench consists of (i) fine-grained video-caption pairs that comprehensively illustrate limb-level dynamics in complex actions, (ii) diverse and challenging question-answer pairs focusing specifically on motion understanding, and (iii) a meticulously curated evaluation set specifically designed to assess hallucination phenomena associated with motion descriptions. Furthermore, to address hallucination issues systematically, we propose the linguistically grounded Motion Parsing and Extraction (MoPE) algorithm, capable of accurately extracting motion-specific attributes directly from textual captions. Leveraging MoPE, we introduce a precise hallucination evaluation metric that functions independently of large-scale vision-language or language-only models. By integrating MoPE into the GRPO post-training framework, we effectively mitigate hallucination problems, significantly improving the reliability of motion-centric video captioning models.

==> sec/5.dataset.tex <==
\section{\model~Dataset}
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/Fig3-SMU-v1.pdf}
\caption{
An example of PaMoR. The motion process description is decomposed into seven core elements: MI (Motion Initiation), AE (Agent Entity), PE (Patient Entity), MM (Magnitude Modifier), DI (Direction Indicator), AQ (Agent Qualifier), and PQ (Patient Qualifier). These elements are expressed using three types of units.
}
\label{fig:unit:case}
\end{figure*}
In this section, we provide a detailed introduction to the proposed \model~dataset and the corresponding standardized construction process.

\subsection{Construction Pipeline}
As illustrated in Figure~\ref{fig:data:pipeline}, the process begins by collecting videos from various sources and segmenting them into clips, each lasting between 5 and 20 seconds.
These video clips are then uniformly sampled into 16 frames.
The preprocessed video frames undergo pose estimation via AlphaPose~\cite{alphapose}, which employs spatiotemporal graph models for robust person ID tracking across frames.

Following the pose annotations, we implement the physical analysis framework detailed in Section~\ref{sec:phy}.
This allows us to extract detailed body movement information for each person in the video, which includes velocity, angular velocity, velocity score, angular velocity score, velocity FFT sequence, angular velocity FFT sequence, and the angle of each joint for every frame., as shown in Figure~\ref{fig:data:pipeline}. 
Such fine-grained motion analysis generates a comprehensive numerical dictionary for each frame, capturing the intricate dynamics of movement.
Subsequently, the physical attributes are embedded into prompts using the template shown in Section~B of the Appendix. 
Six-stage prompting with GPT-4o generates PaMoR-format annotations.
Finally, the PaMoR annotations and original videos undergo multi-modal fusion through the pipeline in Figure~\ref{fig:data:pipeline}, where GPT-4o produces dense captions.
Different from directly employ GPT-4o to generate video captions using single prompt, our pipeline facilitate the generation of dense video captions that provide a detailed representation of the motion process.
\input{tables/data.sta}
\subsection{Statistics}
The \model~Dataset is composed of two distinct components: \model-Caption and \model-Tuple, which are directly aligned with the PaMoR-Caption and PaMoR-Tuple structures, respectively. 
\model-Caption encompasses a comprehensive collection of textual descriptions, amounting to a total of 779,573 words, corresponding to a cumulative video duration of 187 hours. Notably, the dataset exhibits a high level of annotation granularity, with an average of 98.57 annotations per video and an annotation density of 11.56 per second, ensuring a fine-grained and information-rich representation of motion-related events.
